A physical perspective on lithium therapy

Lithium salts have strong medical properties in neurological disorders such as bipolar disorder and lithium-responsive headaches. They have recently gathered attention due to their potential preventive effect in viral infections. Though the therapeutic effect of lithium was documented by Cade in the late 1940s, its underlying mechanism of action is still disputed. Acute lithium exposure has an activating effect on excitable organic tissue and organisms, and is highly toxic. Lithium exposure is associated with a strong metabolic response in the organism, with large changes in phospholipid and cholesterol expression. Opposite to acute exposure, this metabolic response alleviates excessive cellular activity. The presence of lithium ions strongly affects lipid conformation and membrane phase unlike other alkali ions, with consequences for membrane permeability, buffer property and excitability. This review investigates how lithium ions affect lipid membrane composition and function, and how lithium response might in fact be the body's attempt to counteract the physical presence of lithium ions at cell level. Ideas for further research in microbiology and drug development are discussed.

==> ion_transport_R2.tex <==
\begin{itemize}
	
	\item Cells not in equilibrium, modeling of phase transitions and ion transport in MD and theoretically. Topological changes, thermal changes..
	
	\item cortical spreading depression
	
	\item Regulate activity of nerve membrane and mitochondria through phase shift 
	
	\item General on transition in biology: collagen, filament networks. Biopolymers such as collagen, cellular filaments, changes in physical properties such as melting temperature, bulk permeability, persistence length
	
	\item Microdosing \cite{gadh_low-dose_2020}, drinking water \cite{eyre-watt_association_2021}
\end{itemize}
